Similarity-Based Domain Adaptation with LLMs

Unsupervised domain adaptation leverages abundant labeled data from various source domains to generalize onto unlabeled target data. Prior research has primarily focused on learning domain-invariant features across the source and target domains. However, these methods often require training a model using source domain data, which is time-consuming and can limit model usage for applications with different source data. This paper introduces a simple framework that utilizes the impressive generalization capabilities of Large Language Models (LLMs) for target data annotation without the need of source model training, followed by a novel similarity-based knowledge distillation loss. Our extensive experiments on cross-domain text classification reveal that our framework achieves impressive performance, specifically, 2.44\% accuracy improvement when compared to the SOTA method.

==> Figures/main.tex <==
\begin{figure*}[t]
    % \begin{center}
    \centering
\includegraphics[%width=0.6\textwidth
        width=14cm, height=5cm
        ]{crop_figure_1.pdf}
    % \end{center}
    \caption{Proposed framework Overview. LLM is used to construct the source data store, as shown in the upper left corner. Given target data, we first obtain LLM annotations via $k$NN augmented comparison to the data store, then fine-tune an SLM with two training losses: classification consistency loss $\mathcal{L}_1$ and similarity consistency loss $\mathcal{L}_2$.
}
    \label{main}
\vspace{-0.5cm}
\end{figure*}

==> Sections/1_intro.tex <==
\section{Introduction}
Large language models \cite{NEURIPS2020_1457c0d6, NEURIPS2022_b1efde53,workshop2023bloom,openai2023gpt4,touvron2023llama} have demonstrated strong generalization capabilities across a wide range of tasks, indicating their potential as general-purpose models. However, these large language models suffer from efficiency issues due to their size and high inference latency, making them difficult to deploy in real-world applications. Therefore, small models trained on task-specific data are still favored in many resource-constrained scenarios because they have much fewer parameters, are easy to deploy, and perform well in specific downstream tasks. However, fitting a small model for a specific task may require large amounts of human-labeled data, which is not available for many downstream tasks and is expensive to annotate. This data inefficiency problem makes it challenging to fine-tune a small model. Unsupervised Domain Adaptation (UDA) aims to solve this learning problem in the unlabeled target domain by utilizing the abundant knowledge in an existing domain called the source domain, even when these domains may have different distributions \cite{chen-etal-2019-multi-source,karouzos-etal-2021-udalm,miller-2019-simplified}. Current methods often use labeled source data and unlabeled target data to learn domain-invariant and discriminative features \cite{pmlr-v70-saito17a,  du-etal-2020-adversarial, feng2023twostage}. However, this often requires training a model with source data, and the performance of the target model is limited by the original domain model's performance \cite{zhang-etal-2021-matching}. In this paper, we leverage the strong generalization of large language models to address this issue. We propose a SimCross framework, which consists of two training parts. In the first part, we use the $k$-nearest neighbors ($k$NN) method to utilize large language models for annotating target domain data, replacing the previous step of training a domain-generalization model. In the second part, we train a small model on the annotated target domain data, and we also incorporate a novel knowledge distillation (KD) loss to distil the distribution of large language models on target domain data into the small model. We observe that this additional loss can further enhance the small model's learning on the target domain.

In summary, our contributions include:
\begin{itemize}
\setlength{\itemsep}{0pt}
\setlength{\parsep}{0pt}
\setlength{\parskip}{0pt}
\item We propose SimCross, a novel framework that leverages large language models for domain generalization. We demonstrate the effectiveness of our method across multiple domain generalization tasks, with results approaching those obtained with models trained on data with ground truth labels.
\item To more effectively utilize the generalization capabilities of large language models, we introduce a novel loss function to transfer the large model's generalization ability. We conducted extensive experimental analyses to confirm the effectiveness of this loss function.
\end{itemize}

% \section{Research question \& Motivation}
% Most existing  retrieval methods utilize the same model to map both query and retrieved texts to feature vectors, known as symmetric retrieval. To achieve high retrieval accuracy, these methods typically employ a large model for feature extraction, leading to efficiency issues. In practical scenarios with limited computing and memory resources, such as mobile search, deploying a large model for feature extraction on the user side is often impractical, making lightweight models more preferable. One solution is to use lightweight models for both datastore and query feature extraction, but this often results in reduced retrieval accuracy due to the inferior representation capabilities of lightweight models. In asymmetric retrieval settings, where text in the datastore can be processed offline with ample computing resources while queries require feature extraction on end-user devices with limited computing power, it is feasible to use a large model for indexing text and a lightweight model for queries. This approach strikes a balance between retrieval accuracy and efficiency. The core challenge in asymmetric retrieval is the adaptation of lightweight models to map queries into the same embedding space as the text embeddings extracted by large language models.




==> Sections/1_intro_lorraine.tex <==
\section{Introduction}

Unsupervised Domain Adaptation aims to transfer labeled source domain knowledge to the unlabeled target domain. Usually, these domains share common characteristics, for example, book reviews and movie reviews. Typical domain adaptation methods are trained to learn domain invariant features across source and target domains~\cite{pmlr-v70-saito17a,  du-etal-2020-adversarial, feng2023twostage}. 

In spite of their effectiveness, these models are subject to retraining when the domains are changed. The recent generalization ability of large language models (LLMs)~\cite{NEURIPS2020_1457c0d6, NEURIPS2022_b1efde53,workshop2023bloom,openai2023gpt4,touvron2023llama}, raises the question of whether LLMs alone can be used for target domain prediction without retraining. Our paper answers this question using zero/few-shot prompting with only target domain data. Additionally, we demonstrated that the performance improved significantly when k nearest-neighbor (KNN) comparisons were made using the source domain data without training. 

In real-world applications, using LLM for data annotation is costly and prone to efficiency concerns~\cite{openai2023gpt4}. In many resource-constrained scenarios, local models with fewer parameters, i.e small language models (SLMs) and high performance are of great importance. Naive symbolic knowledge distillation methods from LLM into SLM are typically done via supervised training with LLM generations~\cite{west-etal-2022-symbolic}. Inspired by KNN-based LLM prompting, we proposed a novel soft similarity-based distillation loss. Our method includes two components: 1) probability-based distillation loss aiming to match LLM-generated probabilities and 2) similarity-based loss between teacher and student sentence representation distance. 

We present a simple and lightweight framework for distilling cross-domain knowledge without training different source domain models. Using LLMs, we annotate target domain data via $k$NN augmented annotation and train an SLM using a novel knowledge distillation (KD) loss, which not only distills the label distribution of large language models but also provides the SLMs with representation supervision via similarity loss. We show strong knowledge distillation performance improvement using $\text{DistilBERT}_{\text{base}}$ and $\text{BERT}_{\text{base}}$ on eight cross-domain sentiment classification tasks, when compared to multiple baselines. We additionally conducted ablation studies of the proposed framework, revealing the importance of similarity-based annotation and distillation on model performance.

% By assessing LLM-predicted label quality,  the proposed SimLoss, and comparing KL-divergence with cross-entropy loss, w



% Overall, In this paper, we propose a SimCross framework, which consists of two training parts. In the first part, we use the $k$-nearest neighbours ($k$NN) method to utilize large language models for annotating target domain data, replacing the previous step of training a domain-generalization model. In the second part, we train a small model on the annotated target domain data, and we also incorporate a novel knowledge distillation (KD) loss to distil the distribution of large language models on target domain data into the small model. We observe that this additional loss can further enhance the small model's learning on the target domain.

% In summary, our contributions include:
% \begin{itemize}
% \setlength{\itemsep}{0pt}
% \setlength{\parsep}{0pt}
% \setlength{\parskip}{0pt}
% \item We propose SimCross, a novel framework that leverages large language models for domain generalization. We demonstrate the effectiveness of our method across multiple domain generalization tasks, with results approaching those obtained with models trained on data with ground truth labels.
% \item To more effectively utilize the generalization capabilities of large language models, we introduce a novel loss function to transfer the large model's generalization ability. We conducted extensive experimental analyses to confirm the effectiveness of this loss function.
% \end{itemize}

% \lorraine{Work In Progress}

==> Sections/1_intro_wendy.tex <==
\section{Introduction}

Cross-domain sentiment classification aims to classify the text data in new unlabeled target domain based on the labelled text from source domain(s). Usually, these domains share common characteristics, e.g., book reviews and movie reviews, so previous 
% domain adaptation 
classification
methods focus on learning domain invariant features across source and target domains.~\cite{pmlr-v70-saito17a,  du-etal-2020-adversarial, feng2023twostage}.

Despite their effectiveness, these models are subject to retraining when domains are changed. The recent generalization ability of large language models (LLMs)~\cite{NEURIPS2020_1457c0d6, NEURIPS2022_b1efde53,workshop2023bloom,openai2023gpt4,touvron2023llama}, raises the question of whether LLMs alone are good enough for target domain prediction without training. Our paper answers this question using zero/few-shot prompting with examples from source domain. We demonstrated that the performance improved significantly with our $k$ nearest-neighbour ($k$NN) annotation.
% with the $k$ nearest-neighbour ($k$NN) samples from source domain under our . 
% including $k$ nearest-neighbour ($k$NN) samples from source domain into the prompt. 

In real-world applications, deploying LLMs\footnote{We define LLM as language model with at least 7B parameter size.} for sentiment classification is costly and prone to efficiency concerns~\cite{openai2023gpt4}. In many resource-constrained scenarios, local models with fewer parameters, i.e small language models (SLMs) having high performance are of great importance. Naive symbolic knowledge distillation methods from LLM into SLM are typically done via supervised training with LLM generations~\cite{west-etal-2022-symbolic}. 
To effectively train SLMs for cross-domain sentiment classification without training different source domain models, we present a simple and lightweight framework for distilling cross-domain knowledge from LLMs to SLMs.
% we employ KNN-based LLM prompting for target domain annotation, which benefits from the generalizability of LLMs. 
% Inspired by KNN-based LLM prompting, 
% we proposed a novel soft similarity-based distillation loss. Our method includes two components: 1) similarity-based loss aiming to match LLM classification label with SLM and 2) similarity-based loss to align LLM and SLM sentence representation . 

% We present a simple and lightweight framework for distilling cross-domain knowledge without training different source domain models. 
Inspired by $k$NN-LM~\cite{khandelwal20generalization}, we introduce a $k$NN-based annotation that 
performs annotation via $k$ most similar texts from source domain.  
% $k$NN augmented prompting 
We employ knowledge distillation (KD) using the annotation results with a novel similarity-based KD loss. This loss consists of: 1) classification consistency loss aiming to match annotated class labels of target data from LLM with SLM,
% to distil the domain invariant features into SLM 
and 2) similarity consistency loss to align LLM and SLM sentence representation in target domain. 
Since the LLM annotation of target data encoded the information from source domain, we use the former loss to distil domain-invariant features implicitly detected by the generalization ability of LLM. The latter loss is computed based on the batch-wise similarity of target data, which 
% , thus 
distils the domain-aware features from LLM to SLM. 
% which not only distills the label distribution of large language models but also provides the SLMs with representation supervision via similarity loss. 
\input{latex/Figures/main}

We show the effectiveness of our distillation framework using $\text{DistilBERT}_{\text{base}}$ and $\text{BERT}_{\text{base}}$ on eight cross-domain sentiment classification tasks when compared to different models. We additionally conducted ablation study 
% of the proposed framework
, revealing the importance of similarity-based annotation and distillation losses on model performance.

% By assessing LLM-predicted label quality,  the proposed SimLoss, and comparing KL-divergence with cross-entropy loss, w



% Overall, In this paper, we propose a SimCross framework, which consists of two training parts. In the first part, we use the $k$-nearest neighbours ($k$NN) method to utilize large language models for annotating target domain data, replacing the previous step of training a domain-generalization model. In the second part, we train a small model on the annotated target domain data, and we also incorporate a novel knowledge distillation (KD) loss to distil the distribution of large language models on target domain data into the small model. We observe that this additional loss can further enhance the small model's learning on the target domain.

% In summary, our contributions include:
% \begin{itemize}
% \setlength{\itemsep}{0pt}
% \setlength{\parsep}{0pt}
% \setlength{\parskip}{0pt}
% \item We propose SimCross, a novel framework that leverages large language models for domain generalization. We demonstrate the effectiveness of our method across multiple domain generalization tasks, with results approaching those obtained with models trained on data with ground truth labels.
% \item To more effectively utilize the generalization capabilities of large language models, we introduce a novel loss function to transfer the large model's generalization ability. We conducted extensive experimental analyses to confirm the effectiveness of this loss function.
% \end{itemize}

% \lorraine{Work In Progress}

==> Sections/2_related_work.tex <==
 \section{Related Work}

% \noindent\textbf{Unsupervised Domain Adaptation} \quad 
% Unsupervised Domain Adaptation (UDA) is a key technique in machine learning aimed at domain shift problems \cite{ramponi-plank-2020-neural,wright-augenstein-2020-transformer,sheng2021evolving}. Modern UDA strategies primarily focus on two paradigms. The first is centered around learning domain-invariant features, incorporating methods like pivot-based approaches, domain adversarial training, and class-aware feature self-distillation \cite{sun2019unsupervised, 10.1162/tacl_a_00328, ye-etal-2020-feature, wu-shi-2022-adversarial}. The second paradigm utilizes pretrained models to extract task-agnostic features from the target domain and adapts to its subtleties through language modeling~\cite{Du2021CrossDomainGD,karouzos-etal-2021-udalm,feng2023twostage}. \lorraine{@Jie, how does our work compare to the others?}
% These models excel at recognizing and adapting to the unique domain characteristics, enhancing the domain adaptation process.  
% \noindent\textbf{Knowledge Distillation} \quad 
% Knowledge Distillation (KD)~\cite{hinton2015distilling}, involves transferring knowledge from a high-capacity teacher model to a lower-capacity student model through matching the soft targets predicted by the teacher. 
Knowledge Distillation has been employed for domain adaptation, as discussed by \citet{farahani2020brief}. Previous works have focused on distilling domain-invariant knowledge from the teacher model to the student model \cite{hu-etal-2019-domain,ryu2020knowledge, zhang-etal-2021-matching}, which all require extensive training in the source domain.
% Due to the inherent differences between the target and source domains, this often leads to challenges in domain transfer. 
However, our approach of directly utilizing target domain data effectively circumvents this issue.
Symbolic knowledge distillation proposed by \citet{west-etal-2022-symbolic} uses GPT-3 generated data to fine-tune a smaller model. We build on top of this and design a new similarity-based KD loss to distil LLM knowledge to smaller models.
% \lorraine{include symbolic knowledge distillation}

% \subsection{Annotation by Large Language Models}

% Due to the cost and instability of manual labeling, researchers have recently explored using language models for data annotation. \citet{zhang-etal-2021-learning-different}   used the mixup data augmentation framework to assign multiple labels to each example. \citet{wang-etal-2021-want-reduce} investigates using GPT-3 for data annotation. Similarly, \citet{sahu2023promptmix} employs instruction learning to guide large language models to generate and relabel data, while \citet{wang2023lets} extrapolating Errors from Small Models" iteratively guides large language models to generate synthetic datasets with smaller errors compared to real distributions by extrapolating errors from a small model trained on synthesized data against a small real-world validation dataset. Most similar to our work is \cite{saadfalcon2023udapdr}, where large language models are used to generate synthetic queries for reranking tasks. These queries are then used to fine-tune a series of reranking models, which are distilled into a single retriever for adaptation to the target domain. Unlike these methods, we do not require expensive tools like GPT-3 or closed AI; we use open LLMs as effective domain generalization annotation models.



==> Sections/3_method.tex <==

\section{Method}
\input{latex/Tables/main_table}
% Our method revolves around utilizing LLMs for domain generalizable data annotation, which will be used for fine-tuning small models. For data from the target domain, we annotate them by retrieving information from the source domain through LLMs (Section 4.1). After obtaining annotated data for the target domain, we fine-tune the small model and align it with the similarity features of the large model to further improve the performance of the small model (Section 4.2).
% Our method revolves around leveraging the generalization ability of LLM for data annotation in the target domain (\S \ref{sec:method: knn}), and then transferring this domain-generalizable ability to a smaller classification model through distillation. We distill the classification SLM (small language model) in the target domain both with and without the annotated labels as detailed in \S \ref{sec:method:distill}.
% Our method focuses on text classification. 
In this section, we first describe the KNN-based LLM data annotation for target domain (\S \ref{sec:method: knn}), and then introduce the novel knowledge distillation objectives when training SLMs using annotated data from LLMs (\S \ref{sec:method:distill}).

\subsection{$k$NN-based Annotation}
\label{sec:method: knn}
% For cross-domain text classification task, we define a \wendy{labelled} source domain dataset $D_s = \{x_i, y_i\}_{i=1}^m$ with $m$ data samples, and a \wendy{unlabelled} target domain dataset $D_t = \{x_i\}_{i=1}^n$ with $n$ data samples. 
In cross-domain text classification, given labelled examples from source domain $D_s = \{x^s_i, y^s_i\}_{i=1}^m$ with $m$ data samples, the model is tasked to predict labels for the target domain $D_t = \{x^t_i\}_{i=1}^n$ with $n$ examples,
% The goal of cross-domain generalization is to learn a target model $q_t$. 
Considering the feature similarity across domains,  we ask LLMs to compare with source data when annotating target samples. We follow the procedure in $k$NN-LM \cite{khandelwal20generalization}. First, 
each sentence in the source dataset is encoded into a vector representation using LLM, accompanied by its label, we construct a key-value pair $(v^s_i,y^s_i)$ data store as shown in Figure~\ref{main}. Specifically, we append ``It is [MASK].`` to the end of each sentence and use the mask token representation as the key $v^s_i$. The value $y^s_i$ is the original class label.

To annotate the $j$th sentence $x^t_j$ in the target domain, we obtain the masked label embedding $v^t_j$ as above and use this to query the source data store.  We retrieve the $k$ most similar data samples in the source domain by calculating the Euclidean distance $d(v^s_i, v^t_j)$ between the query example and all examples in data store. Lastly, we annotate the target sentence by calculating the weight average across $k$ most similar source data labels, where the weight is proportional to the similarity (normalized negative distance) between the target sentence and the source sentence as shown in equation \ref{eq1}. 
% \begin{equation}
%     P(y^t|v^t_j) \propto \sum\limits_{(v^s_i,y^s_i)\in K_s}  \mathbb{1}_{y^t=y^s_i} \rm{exp}(-d(v^s_i,v^t_j))
%     \label{eq1}
% \end{equation}
\begin{equation}
    P(y^t|v^t_j) \propto \sum\limits_{(v^s_i,y^s_i=y^t)\in K_s}  \rm{exp}(-d(v^s_i,v^t_j))
    \label{eq1}
\end{equation}
where $y^t$ is the possible label space for target domain and $K_s$ denotes the set of $k$ nearest sentences in source domain data store $D_s$. We end up with a distribution over possible labels for the target sentence where we denote to be $p_j$, note that $y^t_j$ is the label with the maximum probability in $p_j$.
\subsection{Distillation Objectives}
\label{sec:method:distill}
Given the target data annotated by LLM, we aim to distill LLM annotation to a SLM. Our proposed distillation method is composed of two parts: classification and batch-wise similarity consistency loss.

\noindent\textbf{Classification Consistency Loss} \quad
The classification consistency loss aims to align the SLM predicted label distribution with the LLM annotated label distribution. For each data sample in $D_t = \{x^t_i, p_i\}_{i=1}^n$, where $p_i$ is the LLM annotated label distribution.
% \footnote{We refer $p^t_i$ to $p_i$ in following context and omit the target notation. We will be referring to target domain in the following content. Same applies to $x_i$.}  
% With the KNN-LLM annotated target dataset $D_t = \{x_i, p_i\}_{i=1}^n$, where $p_i$ is the predicted label distribution, we first fine-tune our model by aligning its prediction distribution of the masked label $q_i$ with the LLM annotated distribution $p_i$. 
we calculate the Kullback–Leibler divergence (KL-divergence) between the SLM predicted distribution $\hat{p}_i$ and the LLM annotated distribution $p_i$, and average the KL-divergence over all the data samples in $D_t$.
% For the target model $f_t$, we optimize it by minimizing the following objective:
\
% $\mathcal{L}_1 = -\frac{1}{n}\sum\limits_{i=1}^n p(x_i)log\frac{p(x_i)}{q_t(x_i)}
\begin{equation}
\label{loss1}
    \mathcal{L}_1 = \frac{1}{n}\sum\limits_{i=1}^n D_{KL}(p_i||\hat{p}_i)
\end{equation}

\noindent\textbf{Similarity consistency loss} \quad
To further transfer the generalization ability of LLM to SLM, we introduce SimLoss which aligns the sentence representation between LLMs and SLMs. Given a batch of $N$ data samples in $D_t$, 
% ${x_i}, i=1,..,N,$, 
we calculate the cosine similarity between the masked label embedding for each example $x_i$ and all the other samples in the same batch using LLM. We then normalize all the similarity values to obtain the distribution of batch-wise cosine similarities for $x_i$, denoted as $s_i$. We repeat the same process for SLM and denote as $\hat{s}_i$ as shown in Equation~\ref{eq:llm_sim}.
% As shown in Equation \ref{eq:llm_sim}, \ref{eq:slm_sim}:
\begin{equation}
\begin{align}
    % S_{l} = [f_{x_i}^Tf_{x_1}, f_{x_i}^Tf_{x_2}, ...,  f_{x_i}^Tf_{x_K}]
    s_i = [s_{1i}, s_{2i}, ..., s_{Ni}]\\
    \hat{s}_i = [\hat{s}_{1i}, \hat{s}_{2i}, ..., \hat{s}_{Ni}]
    \end{align}
 \label{eq:llm_sim}
\end{equation}
where $s_i$ represents the batch-wise similarity distribution derived from LLM, $\hat{s}_i$ represents the one from SLM and $s_{1i}$ denote the normalized similarity between the first and $i$th example in the batch.
% \begin{equation}
    % S_{t} = [f_{x_i}^Tf_{x_1}, f_{x_i}^Tf_{x_2}, ...,  f_{x_i}^Tf_{x_K}]
    % \label{eq:slm_sim}
% \end{equation}

% Then, we convert the similarity into the form of a probability distribution over neighbor anchors.

The SimLoss is computed based on the KL divergence between two probability distributions over all the examples in the batch.
% \begin{equation}
%     p^i = \frac{\mathrm{exp}(S^i)}{\sum_l^K\mathrm{exp}(S^l)}, \mathrm{for}\ i = 1,2,..., K
% \end{equation}
% \begin{equation}
%     \mathcal{L}_2=D_{KL}(p_g||p_{sm})=\sum\limits_{l=1}^{K}p_g^llog\frac{p_q^l}{p_{sm}^l}
% \end{equation}
\begin{equation}
    \mathcal{L}_2=\frac{1}{N}\sum\limits_{i=1}^{N}D_{KL}(s_i||\hat{s}_i)
\end{equation}

The final training loss for the classification SLM is the sum of classification consistency loss and the SimLoss:
$\mathcal{L}=\mathcal{L}_1+\mathcal{L}_2$.
% \section{Concrete Plan}
% I plan to explore knowledge distillation for large retrieval models through two different aspects: one based on a $k$NN \cite{DBLP:journals/corr/abs-1911-00172} architecture and the other focusing on a Ralm \cite{ram2023incontext} architecture. These two approaches differ in how they perform retrieval.

% In the $k$NN-based approach, it is necessary to pre-build a datastore where vectors serve as keys and predicted words as values. During testing, a test example retrieves data from this datastore, and the final prediction is generated by applying softmax to the retrieved set of values.

% On the other hand, the Ralm architecture operates by retrieving examples from the database based on a test example, forming a context, and making predictions under the in-context learning framework (ICL).

% Currently, I have a well-developed plan for knowledge distillation in the $k$NN-based approach, but I have not yet formulated specific ideas for the Ralm architecture.
% \section{Methods}
% For $k$NN-based distillation, we use different training and testing datasets with two significantly different models, such as LLAMA2 7B and Flan-t5-base 250M. The training dataset consists of a series of plain text samples, while the testing dataset comprises natural language questions, like those from SST2 and other classification tasks, transformed into prompts with associated label verbalizations.

% During the training process, we further divide the training dataset into two subsets: $d_{meta-train}$ and $d_{meta-query}$. We pass the $d_{meta-train}$ data through the large model $L$ to obtain the representation $h_{meta-train}$ and $v_{meta-train}$. Similarly, for the $d_{meta-query}$ data, we separately pass it through the large model $L$ to acquire $h_{meta-query}$ and $v_{meta-query}$. Additionally, we process the meta-query data through a smaller model to obtain $h^{small}_{meta-query}$ and $v^{small}_{meta-query}$.

% We then utilize $h_{meta-query}$ to retrieve  from $h_{meta-train}$, essentially computing similarity scores between these vectors. This retrieval process yields the top $k$ (a hyperparameter) results. Formally, 
% \begin{equation}
%     S_l=[h_{query}h_{train}^1,...,h_{query}h_{train}^k]
% \end{equation}
% Simultaneously, we let $h^{small}_{meta-query} $perform retrieval on $h_{meta-train}$, also resulting in the top $k$ results.
% \begin{equation}
%     S_m=[h_{query}^{small}h_{train}^1,...,h_{query}^{small}h_{train}^k]
% \end{equation}
% We compute the  loss by measuring the KL divergence between these two sets of results.
% \begin{equation}
% p_j^i=\frac{exp(S_j^i)/\tau_j}{\sum_{l=1}^{k}exp(S_l^i)/\tau_j}
% \end{equation}
% \begin{equation}
% \mathcal{L}_{KL}^{Retrieval}=D_{KL}(p_l\|\|p_m)
% \end{equation}
% Furthermore, we can obtain probability distributions for the large model's predictions on query examples $pre_{l}$ and the small model's predictions $pre_{m}$. Calculating the KL divergence between these two distributions gives us the second loss.
% \begin{equation}
% \mathcal{L}_{KL}^{Prediction}=D_{KL}(pre_{l}\|\|pre_{m})
% \end{equation}

==> Sections/7_conclusion.tex <==

\section{Conclusion}

In this paper, we propose a novel and simple framework for domain generalization problems. We annotate cross-domain data with large language models and distill the similarity consistency of large language models during the fine-tuning process of small models. We transfer the domain generalization knowledge of large language models to small models like BERT and DistillBERT. Our method defeats the latest domain generalization methods and achieves near ground truth fine-tuning results, making it a promising method for cross-domain classification adaptation.

\section*{Limitation}

Firstly, we only consider one open-source large model, mistral, in our framework. It is necessary to test our method on a broader range of open-source models to understand the domain generalization capabilities of different large language models.

Secondly, we assume that LLMs have rich domain generalization knowledge for specific tasks, but there is no guarantee in real-world applications. This might be addressed through instruction tuning to give LLMs a deeper understanding of the tasks they need to solve.

Thirdly, our research focuses only on sentiment classification tasks. Other natural language processing tasks also face similar challenges, such as cross-domain entity recognition. Therefore, future research should aim to evaluate the applicability of our method to other tasks.

